Select, Extract and Generate: Neural Keyphrase Generation with Layer-wise Coverage Attention

Natural language processing techniques have demonstrated promising results in keyphrase generation. However, one of the major challenges in \emph{neural} keyphrase generation is processing long documents using deep neural networks. Generally, documents are truncated before given as inputs to neural networks. Consequently, the models may miss essential points conveyed in the target document. To overcome this limitation, we propose \emph{SEG-Net}, a neural keyphrase generation model that is composed of two major components, (1) a selector that selects the salient sentences in a document and (2) an extractor-generator that jointly extracts and generates keyphrases from the selected sentences. SEG-Net uses Transformer, a self-attentive architecture, as the basic building block with a novel \emph{layer-wise} coverage attention to summarize most of the points discussed in the document. The experimental results on seven keyphrase generation benchmarks from scientific and web documents demonstrate that SEG-Net outperforms the state-of-the-art neural generative methods by a large margin.

==> sections/background.tex <==
\section{Background}
\label{sec:arch}
% \cite{vaswani2017attention}
SEG-Net uses a Transformer as the building block that consists of stacked encoder and decoder layers.
Each encoder and decoder layer consists of two and three sublayers, respectively.
An encoder layer is composed of multi-head attention, followed by a position-wise feed-forward layer.
A decoder layer has two consecutive multi-head attention layers followed by a position-wise feed-forward layer.
% The multi-head attention employed in Transformer is based on the self-attention mechanism where each element in an input sequence attends to every other element of the input, including itself while computing the output representation.
In the first multi-head attention sublayer, the decoder uses masking in its self-attention to prevent an element from incorporating information about future elements during training.
% This is analogous to the \emph{unidirectional} RNN that is employed as a decoder in a recurrent sequence-to-sequence network.
The second attention sublayer in a decoder layer applies self-attention between the encoded input sequence and each element of the decoded sequence.
% This attention sublayer is akin to the encoder-decoder attention in sequence-to-sequence learning \cite{bahdanau2014neural,luong2015effective}.
Each encoder and decoder layer uses residual connections followed by layer normalization around each sublayer.
% The encoder-decoder layer of the Transformer is depicted in Figure \ref{fig:reader}.

% The Transformer consists of stacked multi-head attention and parameterized linear transformation layers for both the encoder and decoder.


% \subsection{Multi-head Attention}
% \label{sec:multi-head}
% In multi-head attention, there are $h$ identical attention heads that employ the self-attention mechanism.
% In each attention head, a sequence of input vectors, $\mathbf{x}=(x_1, \dots, x_n)$ where $x_i \in R^{d_{model}}$ are transformed into a sequence of output vectors, $\mathbf{o}=(o_1, \dots, o_n)$ where $o_i \in R^{d_k}$ as:
% \begin{gather*}
% \label{eq:mulhead}
% o_i = \sum^{n}_{j=1} \alpha_{ij} \left( x_j W^V \right), \\
% e_{ij} = \frac{x_i W^Q \left( x_j W^K \right)^T}{\sqrt{d_k}},\ \alpha_{ij} = \frac{\exp(e_{ij})}{\sum^{n}_{k=1} \exp(e_{ik})},
% \end{gather*}
% where the parameters $W^Q, W^K \in R^{d_{model} \times d_k}$ and $W^V \in R^{d_{model} \times d_v}$ are unique per attention head.


% \smallskip\noindent
\subsection{Position Representations}
Transformer neither employs recurrence nor convolution. Hence, we need to inject either absolute or relative position of the tokens in a sequence explicitly to make use of the order information.
In the SEG-Net, we employ absolute and relative position representation during encoding the input document and decoding the keyphrases, respectively.

\smallskip\noindent
\textbf{Absolute Position Representations}
We train an embedding matrix $W_{posi}$ that learns to encode tokens' absolute positions in a document into vectors of dimension $d_{model}$.

\smallskip\noindent
\textbf{Relative Position Representations}
\label{subsec:rel_pos_desc}
Since we aim to generate a \emph{set} of keyphrases, the order of their generation should not matter.
Hence, we want the decoder to learn the pairwise relationships between the keyphrases instead of a specific ordering.
% such as alphabetical or length-based ordering.
To encode the pairwise relationships between input elements, we adopt the relative position representations as suggested in \citet{shaw-etal-2018-self}.
% To encode the pairwise relationships between input elements, \citet{shaw2018self} extended the self-attention mechanism as follows.

% \begin{align*}
% o_i & = \sum^{n}_{j=1} \alpha_{ij} \left( x_j W^V + a_{ij}^V \right), \\
% e_{ij} & = \frac{x_i W^Q \left( x_j W^K + a_{ij}^K \right)^T}{\sqrt{d_k}},
% \end{align*}
% where, $a_{ij}^V$ and $a_{ij}^K$ are relative positional representations for the two position $i$ and $j$.
% \cite{shaw2018self} suggested clipping the maximum relative position to a maximum absolute value of $k$.
% \begin{equation*}
% a_{ij}^K = w_{clip(j-i, k)}^K,\ a_{ij}^V = w_{clip(j-i, k)}^V,
% \end{equation*}
% \begin{equation*}
% % \vspace{-2mm}
% clip(x, k) = \max(-k, \min(k, x)).
% \end{equation*}
% We learn $2k+1$ position representations: $w^K=(w_{-k}^K, \dots, w_k^K)$, and $w^V=(w_{-k}^V, \dots, w_k^V)$.


\subsection{Layer-wise Coordination}
\label{subsec:layerwise-coord}
In Transformer, the stacked encoder layers generate a sequence of output vector representations for the source sequence layer by layer, gradually from the lowest layer to the highest layer.
Then each layer of the decoder takes the last layer (the highest layer) representations from the encoder as inputs while computing the output representations for each position in the target sequence.
In essence, all the layers in the decoder attend the output representations produced by the last layer of the encoder.
% This design choice  makes it challenging to apply the coverage mechanism \cite{tu2016modeling,chen2018keyphrase}.
% Hence, we adopt the layer-wise coordination technique \cite{he2018layer} in Transformer.
According to layer-wise coordination, the $i$-th layer of the decoder generates output representations for a target token based on $(i-1)$-th layer's output representations of that token and its preceding tokens and the output representation for all the source tokens from the $i$-th layer of the encoder. 
In simpler words, with the same number of encoder and decoder layers, the output representation produced by a decoder layer depends on the output representations provided by the corresponding encoder layer and the previous layer of the decoder.
Although, incorporation of the layer-wise coordination requires the same number of layers in encoder and decoder, it has a couple of advantages. 
First, it enables us to incorporate the coverage mechanism at each layer.
Second, presumably the lower and higher layers of encoder and decoder encodes syntactic and semantic features, respectively.
% Hence, we adopt the layer-wise coordination technique in SEG-Net.
% Hence, we combine keyphrases and their part-of-speech tag sequence generation based on the higher and lower layers' output representation through multi-task learning.
% Note that the incorporation of the layer-wise coordination requires the same number of layers in encoder and decoder. 


==> table/akp_result.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
% \resizebox{\linewidth}{!}{%
% \small
% \begin{tabular}{l|c@{\hskip 0.125in} c@{\hskip 0.125in} c|c@{\hskip 0.125in} c@{\hskip 0.125in} c}
\begin{tabular}{l|c c| c c|c c|c c|c c}
\hline
\hline
\multirow{ 2}{*}{Model} & \multicolumn{2}{c|}{KP20k} & \multicolumn{2}{c|}{Inspec} & \multicolumn{2}{c|}{Krapivin} & \multicolumn{2}{c|}{NUS} & \multicolumn{2}{c}{SemEval} \\ 
\cline{2-11}
& F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 \\ 
\hline
\hline
% \multicolumn{7}{l}{Prior Works} \\
% \hline
catSeq \cite{yuan2018one} & 0.032 & 0.015 & 0.008 & 0.004 & 0.036 & 0.018 & 0.028 & 0.016 & 0.028 & 0.020 \\
catSeqD \cite{yuan2018one} & 0.031 & 0.015 & 0.011 & 0.007 & 0.037 & 0.018 & 0.024 & 0.014 & 0.024 & 0.016 \\
catSeqCorr \cite{chen2018keyphrase} & 0.032 & 0.015 & 0.009 & 0.005 & 0.038 & 0.020 & 0.024 & 0.014 & 0.026 & 0.018 \\
catSeqTG \cite{chen2019guided} & 0.032 & 0.015 & 0.011 & 0.005 & 0.034 & 0.018 & 0.018 & 0.011 & 0.027 & 0.019 \\
\hline
SEG-Net (This work) & \textbf{0.038} & \textbf{0.019} & \textbf{0.014} & \textbf{0.009} & \textbf{0.056} & \textbf{0.028} & 0.020 & 0.012 & \textbf{0.031} & 0.021 \\
\hline
\end{tabular}
% }
\vspace{2mm}
\caption{Results of absent keyphrase generation on the five keyphrase benchmarks.
The paired t-test is conducted by comparing the best and second-best models under each metric, and the test result is presented in bold-faced (p-value < 0.05).
}
% }
\label{result:absent}
\vspace{-5mm}
\end{table*}


==> table/main_result_v0.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{%
\small
% \begin{tabular}{l|c@{\hskip 0.125in} c@{\hskip 0.125in} c|c@{\hskip 0.125in} c@{\hskip 0.125in} c}
\begin{tabular}{l|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
% \begin{tabular}{l|c c|c c|c c|c c|c c}
% \hline
\hline
\multirow{ 2}{*}{Model} & \multicolumn{2}{c|}{KP20k} & \multicolumn{2}{c|}{Inspec} & \multicolumn{2}{c|}{Krapivin} & \multicolumn{2}{c|}{NUS} & \multicolumn{2}{c}{SemEval} \\
\cline{2-11}
& F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 \\ 
\hline
% \hline
\multicolumn{11}{l}{Present Keyphrase Generation} \\
\hline
catSeq &  0.367 & 0.291 & 0.262 & 0.225 & 0.354 & 0.269 & 0.397 & 0.323 & 0.283 & 0.242 \\
catSeqD & 0.363 & 0.285 & 0.263 & 0.219 & 0.349 & 0.264 & 0.394 & 0.321 & 0.274 & 0.233 \\
catSeqCorr  & 0.365 & 0.289 & 0.269 & 0.227 & 0.349 & 0.265 & 0.390 & 0.319 & 0.290 & 0.246 \\
catSeqTG  & 0.366 & 0.292 & 0.270 & 0.229 & 0.366 & 0.282 & 0.393 & 0.325 & 0.290 & 0.246 \\
Transformer &  0.368 & 0.291 & 0.264 & 0.225 & 0.356 & 0.274 & 0.405 & 0.328 & 0.288 & 0.245 \\
SEG-Net & \textbf{0.381}$^\dagger$ & \textbf{0.323}$^\dagger$ & \textbf{0.301}$^\dagger$ & \textbf{0.246}$^\dagger$ & \textbf{0.378}$^\dagger$ & \textbf{0.299}$^\dagger$ & \textbf{0.459}$^\dagger$ & \textbf{0.401}$^\dagger$ & \textbf{0.341}$^\dagger$ & \textbf{0.298}$^\dagger$ \\
\hline
\multicolumn{11}{l}{Absent Keyphrase Generation} \\
\hline
catSeq & 0.032 & 0.015 & 0.008 & 0.004 & 0.036 & 0.018 & \textbf{0.028}$^\dagger$ & \textbf{0.016} & 0.028 & 0.020 \\
catSeqD & 0.031 & 0.015 & 0.011 & 0.006 & 0.037 & 0.018 & 0.024 & 0.015 & 0.024 & 0.016 \\
catSeqCorr  & 0.032 & 0.015 & 0.009 & 0.005 & 0.038 & 0.020 & 0.024 & 0.014 & 0.026 & 0.018 \\
catSeqTG  & 0.032 & 0.015 & 0.011 & 0.005 & 0.034 & 0.018 & 0.018 & 0.011 & 0.027 & 0.019 \\
Transformer & 0.031 & 0.015 & 0.009 & 0.005 & 0.038 & 0.020 & \textbf{0.028}$^\dagger$ & \textbf{0.016} & 0.029 & 0.020 \\
SEG-Net & \textbf{0.038}$^\dagger$ & \textbf{0.020}$^\dagger$ & \textbf{0.014}$^\dagger$ & \textbf{0.009}$^\dagger$ & \textbf{0.056}$^\dagger$ & \textbf{0.028}$^\dagger$ & 0.024 & 0.014 & \textbf{0.031} & \textbf{0.021} \\
\hline
\end{tabular}
}
\vspace{-2mm}
\caption{
Results of keyphrase prediction on the five scientific benchmarks.
The bold-faced values indicate the best performances across the board.
$^\dagger$ means the model is statistically significantly better (by paired bootstrap test, $p < 0.05$) than all other models.
% The paired t-test is conducted by comparing the best and second-best models under each metric, and the test result is presented in bold-faced (p-value < 0.05).
}
% }
\label{result:main}
\vspace{-2mm}
\end{table*}


==> table/pkp_result.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
% \resizebox{\linewidth}{!}{%
% \small
% \begin{tabular}{l|c@{\hskip 0.125in} c@{\hskip 0.125in} c|c@{\hskip 0.125in} c@{\hskip 0.125in} c}
\begin{tabular}{l|c c|c c|c c|c c|c c}
\hline
\hline
\multirow{ 2}{*}{Model} & \multicolumn{2}{c|}{KP20k} & \multicolumn{2}{c|}{Inspec} & \multicolumn{2}{c|}{Krapivin} & \multicolumn{2}{c|}{NUS} & \multicolumn{2}{c}{SemEval} \\ 
\cline{2-11}
& F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 \\ 
\hline
\hline
% \multicolumn{7}{l}{Prior Works} \\
% \hline
catSeq &  0.367 & 0.291 & 0.262 & 0.225 & 0.354 & 0.269 & 0.397 & 0.323 & 0.283 & 0.242 \\
catSeqD & 0.363 & 0.285 & 0.263 & 0.219 & 0.349 & 0.264 & 0.394 & 0.321 & 0.274 & 0.233 \\
catSeqCorr & 0.365 & 0.289 & 0.269 & 0.227 & 0.349 & 0.265 & 0.390 & 0.319 & 0.290 & 0.246 \\
catSeqTG & 0.366 & 0.292 & 0.270 & 0.229 & 0.366 & 0.282 & 0.393 & 0.325 & 0.290 & 0.246 \\
\hline
SEG-Net (This work) & \textbf{0.381} & \textbf{0.323} & \textbf{0.301} & \textbf{0.246} & 0.368 & \textbf{0.299} & \textbf{0.459} & \textbf{0.401} & \textbf{0.341} & \textbf{0.298} \\
\hline
\end{tabular}
% }
% \vspace{2mm}
\caption{
Results of present keyphrase extraction on the five keyphrase benchmarks.
The paired t-test is conducted by comparing the best and second-best models under each metric, and the test result is presented in bold-faced (p-value < 0.05).
}
% }
\label{result:present}
% \vspace{-5mm}
\end{table*}

